SrTR: Self-reasoning Transformer with Visual-linguistic Knowledge for Scene Graph Generation

Objects in a scene are not always related. The execution efficiency of the one-stage scene graph generation approaches are quite high, which infer the effective relation between entity pairs using sparse proposal sets and a few queries. However, they only focus on the relation between subject and object in triplet set subject entity, predicate entity, object entity, ignoring the relation between subject and predicate or predicate and object, and the model lacks self-reasoning ability. In addition, linguistic modality has been neglected in the one-stage method. It is necessary to mine linguistic modality knowledge to improve model reasoning ability. To address the above-mentioned shortcomings, a Self-reasoning Transformer with Visual-linguistic Knowledge (SrTR) is proposed to add flexible self-reasoning ability to the model. An encoder-decoder architecture is adopted in SrTR, and a self-reasoning decoder is developed to complete three inferences of the triplet set, s+o-p, s+p-o and p+o-s. Inspired by the large-scale pre-training image-text foundation models, visual-linguistic prior knowledge is introduced and a visual-linguistic alignment strategy is designed to project visual representations into semantic spaces with prior knowledge to aid relational reasoning. Experiments on the Visual Genome dataset demonstrate the superiority and fast inference ability of the proposed method.

==> proposed2.tex <==

\begin{figure*}[tp] \small
	\vspace{-2em}
	\begin{center}
		\centering
		%		\begin{tabular}{cc}
		\epsfig{width=2.2\figurewidth,file=Figures/LDGnet.png}
		%		\end{tabular}
		%		\vspace*{-0.1in}
		\caption{\label{fig:Flowchart}
			Flowchart of the proposed LDGnet, including an image encoder, a text encoder, and a visual-linguistic alignment employing learning domain invariant representation. Red, green and blue represent three classes respectively. In the semantic space, dots represent visual features and pentagon represents linguistic features.}
	\end{center}
	\vspace{-2em}
\end{figure*}

Notations used in this paper is summarized in Table \ref{table:Notations}. Assume that ${{\bf{X}}} = \left\{ {{\bf{x}}_i} \right\}_{i = 1}^{{N}}\in\mathbb{R}{^d}$ is the data from SD, and ${{\bf{Y}}}= \left\{ {{\bf{y}}_i} \right\}_{i = 1}^{{N}}$ is the corresponding class labels. Here, $d$ and $N$ denote the dimension of data and the number of source samples, respectively. The proposed LDGnet is broken into three parts: an image encoder, a text encoder, and a visual-linguistic alignment. The flowchart for each part is illustrated in Fig.~\ref{fig:Flowchart}. The sample of 13$\times $13$\times d$ spatial patch in HSI is selected from SD, and each one is assigned a coarse-grained text and two fine-grained texts based on the class of the patch. In the visual mode, the image is delivered to the image encoder to extract features, and then the classification head $C$ is used to calculate the cross entropy loss, and the projection head $P$ outputs visual features for visual-linguistic alignment. To extract the linguistic features and create the cross-domain shared semantic space, the text is passed to the text encoder. Finally, supervised contrastive learning is used for visual-linguistic alignment to align image and text by class.


\subsection{Image encoder}

Given that HSI is a 3D data cube made up of hundreds of spectral channels with a wealth of spatial and spectral information, the Deep residual 3D CNN network is used to extract spatial-spectral features, as shown in Fig.~\ref{fig:image}. The image encoder is made up of two 3D residual Block-MaxPool3d modules and one Conv3d module, where the 3D residual Block serving as the core module for extracting robust visual features. The 3D residual Block is composed of two Conv3d-BN3d-ReLUs and one Conv3d in series. The output of the first Conv3d-BN3d-ReLU and the output of Conv3d are used for residual connection. The extracted spatial-spectral features are sent to the classification head $Cls$ and the cross entropy is calculated with the ground truth. At the same time, it is fed into the projection head $Proj$ to obtain the visual features for feature alignment of visual modes and linguistic modes. The cross-entropy loss is defined as,
\begin{equation}\label{eq:11}
{{\cal L}_{ce}}\left( {{{\bf{p}}_i},{{\bf{y}}_i}} \right) =  - \sum\limits_c {y_i^c\log p_i^c} 
\end{equation}
where ${\bf{y}}_i$ is the one-hot encoding of the label information of ${{\bf{x}}_i}$, $c$ is the index of class, and ${{\bf{p}}_i}$ is the predicted probability output obtained by $Cls$. Therefore, the classification loss for SD is defined as,
\begin{equation}\label{eq:12}
{{{\cal L}_{SD}}\left( {{\bf{X}},{\bf{Y}}} \right) = \frac{1}{N}\sum\limits_i {{{\cal L}_{ce}}\left( {C\left( {{{\bf{x}}_i}} \right),{{\bf{y}}_i}} \right).} }
\end{equation}

\begin{figure*}[tp] \small
	\begin{center}
		\centering
		\epsfig{width=1.6\figurewidth,file=Figures/image encoder.png}
		\caption{\label{fig:image}
			The flowchart of image encoder, where the 3D residual Block is the primary module.}
	\end{center}
	\vspace{-2em}
\end{figure*}

\subsection{Text encoder}

The text encoder is a language-model transformer \cite{vaswani2017attention} modified in accordance with Radford et al. \cite{radford2019language}. The text encoder start with a base size of a 33M-parameter, 3-layer, 512-wide model with 8 attention heads. Similar to CLIP, the text is represented by the transformer using a lower-cased byte pair encoding (BPE) with a vocabulary size of 49,152 \cite{sennrich2016neural}. The maximum sequence length is limited to 76 for computational efficiency. The \textcolor[rgb]{0.3,0.3,0.3}{\sffamily [SOS]} and \textcolor[rgb]{0.3,0.3,0.3}{\sffamily [EOS]} tokens are used to bracket the text sequence, and the activations of the highest layer of the transformer at the \textcolor[rgb]{0.3,0.3,0.3}{\sffamily [EOS]} token are treated as the linguistic feature of the text. This linguistic feature is then normalized by layer and linearly projected into the semantic space.

According to the prior knowledge of land cover classes in SD scene, coarse-grained and fine-grained text descriptions are assigned to each land cover classes. As shown in Fig.~\ref{fig:prompt}, \textcolor[rgb]{0.3,0.3,0.3}{\sffamily A hyperspectral image of \textless class name\textgreater} is used as a template to construct coarse-grained text descriptions for each class in a cloze way. As for fine-grained text, combined with prior knowledge, the color, shape, distribution and adjacency relationship are described manually, such as \textcolor[rgb]{0.3,0.3,0.3}{\sffamily The grass stress is pale green}, \textcolor[rgb]{0.3,0.3,0.3}{\sffamily The trees beside road} and \textcolor[rgb]{0.3,0.3,0.3}{\sffamily The road appears as elongated strip shape}. Each land cover class sets two fine-grained text, the hollow pentagon shown in Fig.~\ref{fig:prompt}.

\begin{figure}[tp] \small
	\begin{center}
		\centering
		\epsfig{width=1.10\figurewidth,file=Figures/prompt.png}
		\caption{\label{fig:prompt}
			Examples of coarse-grained and fine-grained text for three classes.}
	\end{center}
	\vspace{-2em}
\end{figure}

\subsection{Visual-linguistic alignment}

The linguistic features obtained by text encoder construct semantic space as a cross-domain shared space. To achieve the alignment of visual features and linguistic features by class, supervised comparative learning is performed, and the domain invariant representation driven by language is developed to generalize the model to TD. Firstly, a supervised contrastive learning is defined as follow,
\begin{equation}\label{eq:1}
{{\cal L}_{supcon}} =  - \sum\limits_{i = 0}^N {\frac{1}{{|P(i)|}}} \sum\limits_{p \in P(i)} {\log } \frac{{\exp \left( {{{{\bf{x}}_i^T{\bf{x}}_p^ + } \mathord{\left/
					{\vphantom {{{\bf{x}}_i^T{\bf{x}}_p^ + } \tau }} \right.
					\kern-\nulldelimiterspace} \tau }} \right)}}{{\sum\limits_{a \in A(i)} {\exp \left( {{{{\bf{x}}_i^T{\bf{x}}_a^ - } \mathord{\left/
						{\vphantom {{{\bf{x}}_i^T{\bf{x}}_a^ - } \tau }} \right.
						\kern-\nulldelimiterspace} \tau }} \right)} }}
\end{equation}
where for each embedding feature ${{\bf{x}}_i}$ in minibatch, ${P(i)}$ and ${A(i)}$ are the positive and negative sample sets, ${|P(i)|}$ is the number of positive samples, ${{\bf{x}}_p^ + }$ and ${{\bf{x}}_a^ - }$ are one of the positive and negative samples. 

Given a batch of $bs$ image-text pairs with the same label, the alignment losses ${{\cal L}_{supcon}}$ of image to text and text to image are calculated,
\begin{equation}\label{eq:2}
\begin{array}{l}
{{\cal L}_{coarse}} =  - \sum\limits_{i = 0}^N {\frac{1}{{|P(i)|}}} (\sum\limits_{p \in {P_l}(i)} {\log } \frac{{\exp ({{{\bf{v}}_i^T{\bf{l}}_p^ + } \mathord{\left/
				{\vphantom {{{\bf{v}}_i^T{\bf{l}}_p^ + } \tau }} \right.
				\kern-\nulldelimiterspace} \tau })}}{{\sum\limits_{a \in {A_l}(i)} {\exp ({{{\bf{v}}_i^T{\bf{l}}_a^ - } \mathord{\left/
					{\vphantom {{{\bf{v}}_i^T{\bf{l}}_a^ - } \tau }} \right.
					\kern-\nulldelimiterspace} \tau })} }}\\
\begin{array}{*{20}{c}}
{}&{}&{}
\end{array} + \sum\limits_{p \in {P_v}(i)} {\log } \frac{{\exp {{({\bf{l}}_i^T{\bf{v}}_p^ + } \mathord{\left/
				{\vphantom {{({\bf{l}}_i^T{\bf{v}}_p^ + } \tau }} \right.
				\kern-\nulldelimiterspace} \tau })}}{{\sum\limits_{a \in {A_v}(i)} {\exp ({{{\bf{l}}_i^T{\bf{v}}_a^ - } \mathord{\left/
					{\vphantom {{{\bf{l}}_i^T{\bf{v}}_a^ - } \tau }} \right.
					\kern-\nulldelimiterspace} \tau })} }})
\end{array}
\end{equation}
where for each visual feature ${{\bf{v}}_i}$ and linguistic feature ${{\bf{l}}_i}$ in minibatch, ${{P_v}(i)}$ and ${{A_v}(i)}$ are the positive and negative sample sets of visual feature, ${{P_l}(i)}$ and ${{A_l}(i)}$ are the positive and negative sample sets of linguistic feature, ${|{P_v}(i)|=|{P_l}(i)|=|P(i)|}$. In addition, the temperature parameter $\tau$, which governs the range of the logits in the softmax, is explicitly optimized as a log-parameterized multiplicative scalar during training. ${\cal L}_{coarse}$ represents the alignment loss of image to coarse-grained text. The alignment loss of image to fine-grained text ${\cal L}_{fine}$ is similar to it, with the difference being that linguistic features require two fine-grained linguistic features. In the process of optimizing, the visual features and linguistic features belonging to the same class are put into ${{P_v}(i)}$ and ${{P_l}(i)}$, and the features outside the class are put into ${{A_v}(i)}$ and ${{A_l}(i)}$. The image encoder and text encoder are optimized by${\cal L}_{coarse}$ and ${\cal L}_{fine}$ to bring features from the same class closer together and samples from different classes farther apart. This allows image encoder to learn class-specific domain invariant representations.

In LDGnet, the image encoder and text encoder are jointly trained. Integrating above loss functions, the total loss of LDGnet is defined as follows,
\begin{equation}\label{eq:17}
{{\cal L}_{total}} = {{\cal L}_{SD}} + \lambda \left( {\left( {1 - \alpha } \right){{\cal L}_{coarse}} + \alpha {{\cal L}_{fine}}} \right)
\end{equation}
where $\lambda$ is a hyper-parameter for balancing the alignment loss, and $\alpha$ is employed to control the contribution of both coarse- and fine-grained linguistic features. 

\subsection{Generalization Performance of LDGnet}
In SDEnet, the generator $G$ is required to produce ED with domain-specific information (domain shift with SD) and domain invariant discriminat information, while the discriminator $D$ is expected to extract class-wise domain invariant representations from SD, ID and ED. We take the Houston dataset as an example to illustrate $G$ and $D$. As shown in Fig. \ref{fig:analysis}(a) original samples from SD, and ED output by $G$, and (b) SD features and ED features output by $P$, where SD is the Houston 2013 data, $\bullet$ represents SD, × represents ED, and the number represents class index. It can be seen from Fig. \ref{fig:analysis}(a), for instance, in the 1-st class, 2-nd class and 3-rd class, there is a certain domain shift between SD and ED of the same class (the same color). Further, the samples of the same class in ED are aggregated better, indicating that they maintain the discriminant information in SD. It is obvious that $D$ extracts the class-wise domain invariant representation, as shown in Fig. \ref{fig:analysis}(b), where $D$ effectively alleviates the domain shift between SD and ED during training. In addition, the MMD distance between SD and ED of the original samples and features output by $P$ are quantitatively analyzed in Table \ref{table:analysis}. There is a distribution gap of about 0.78 between ED and SD in each class, and the gap is reduced by about 0.6 after obtaining embedding features through $D$. This also indicates that $G$ and $D$ in SDEnet perform their duties well and learn the class-wise domain invariant representation.

The TD (Houston 2018 data) is inferred directly by fully trained SDEnet. The visualization of class separability in the original space and feature space are shown in Fig. \ref{fig:analysis}(c) and (d). The inter-class distribution is mixed together in Fig. \ref{fig:analysis}(c), and the separability is significantly improved after feature embedding by SDEnet. In Fig. \ref{fig:analysis}(d), the inter-class distance is obviously increased and the intra-class distance is reduced. This shows that SDEnet has the ability to extract class-wise domain invariant representations and is well generalized to TD by learning the differences between SD, ID and ED. In addition, it can be seen from the $mmd(SD,TD)$ in Table \ref{table:analysis} that the original distribution gap between SD and TD is also decreased by about 0.1 in the feature space of SDEnet output.
\begin{table}[]
		\caption{\label{table:analysis}
	The MMD distance between SD and ED and between SD and TD of the original samples and features output by $P$. \\ (Houston dataset)}
	\begin{center}
	\begin{tabular}{|c|cc|cc|}
		\hline \hline
		\multirow{2}{*}{Class} & \multicolumn{2}{c|}{$mmd(SD,ED)$}              & \multicolumn{2}{c|}{$mmd(SD,TD)$}              \\ \cline{2-5} 
		& \multicolumn{1}{c|}{origin} & projection & \multicolumn{1}{c|}{origin} & projection \\ \hline
		1                    & \multicolumn{1}{c|}{0.7881} & 0.1671     & \multicolumn{1}{c|}{0.4870} & 0.3723     \\
		2                    & \multicolumn{1}{c|}{0.7854} & 0.1753     & \multicolumn{1}{c|}{0.4386} & 0.3189     \\
		3                    & \multicolumn{1}{c|}{0.7882} & 0.1620     & \multicolumn{1}{c|}{0.4126} & 0.3239     \\
		4                    & \multicolumn{1}{c|}{0.7579} & 0.1819     & \multicolumn{1}{c|}{0.3610} & 0.2909     \\
		5                    & \multicolumn{1}{c|}{0.8056} & 0.1729     & \multicolumn{1}{c|}{0.4657} & 0.3474     \\
		6                    & \multicolumn{1}{c|}{0.7661} & 0.1789     & \multicolumn{1}{c|}{0.4088} & 0.3193     \\
		7                    & \multicolumn{1}{c|}{0.7863} & 0.1758     & \multicolumn{1}{c|}{0.4212} & 0.3301     \\ \hline
		Mean                 & \multicolumn{1}{c|}{0.7825} & \textbf{0.1734}     & \multicolumn{1}{c|}{0.4278} & \textbf{0.3290}     \\ \hline \hline
	\end{tabular}
	\end{center}
\vspace{-2em}
\end{table}


